Influence Functions for Scalable Data Attribution in Diffusion Models

Diffusion models have led to significant advancements in generative modelling. Yet their widespread adoption poses challenges regarding data attribution and interpretability. In this paper, we aim to help address such challenges in diffusion models by developing an influence functions framework. Influence function-based data attribution methods approximate how a model's output would have changed if some training data were removed. In supervised learning, this is usually used for predicting how the loss on a particular example would change. For diffusion models, we focus on predicting the change in the probability of generating a particular example via several proxy measurements. We show how to formulate influence functions for such quantities and how previously proposed methods can be interpreted as particular design choices in our framework. To ensure scalability of the Hessian computations in influence functions, we systematically develop K-FAC approximations based on generalised Gauss-Newton matrices specifically tailored to diffusion models. We recast previously proposed methods as specific design choices in our framework and show that our recommended method outperforms previous data attribution approaches on common evaluations, such as the Linear Data-modelling Score (LDS) or retraining without top influences, without the need for method-specific hyperparameter tuning.

==> sections/experiments--maybe-include-these.tex <==



\begin{figure}[!htb]
    \centering
    \includegraphics{figures/gradient_norms_losses.pdf}
    \caption{Caption}
    \label{fig:cifar2-measurement-gradient-norms}
\end{figure}
\begin{figure}[!htb]
    \centering
    \includegraphics{figures/gradient_norms_losses_per_timestep.pdf}
    \caption{Measurement gradient norms and gradient deviations for the diffusion losses at different timesteps as per \Cref{eq:per-timestep-loss}. Individual markers represent averages for measurements on a single sampled datapoint.}
    \label{fig:cifar2-measurement-gradient-norms-per-timestep}
\end{figure}


\begin{figure}[!htb]
    \centering
     \begin{subfigure}[b]{1.0\textwidth}
         \centering
         \includegraphics[width=\textwidth,trim={0cm 0.7cm 0 0.0cm},clip]{figures/measurement_lin/meas_linearisation_analysis_target_10_this_retrain_idxs_id_0.pdf}
     \end{subfigure}
     \begin{subfigure}[b]{1.0\textwidth}
         \centering
         \includegraphics[width=\textwidth,trim={0cm 0.7cm 0 0.8cm},clip]{figures/measurement_lin/meas_linearisation_analysis_target_10_this_retrain_idxs_id_1.pdf}
     \end{subfigure}
     \begin{subfigure}[b]{1.0\textwidth}
         \centering
         \includegraphics[width=\textwidth,trim={0cm 0.0cm 0 0.8cm},clip]{figures/measurement_lin/meas_linearisation_analysis_target_10_this_retrain_idxs_id_2.pdf}
     \end{subfigure}
    % \includegraphics[width=0.5\linewidth]{}
    \caption{Predicted change in diffusion loss $\mathcal{L}_t$ at different timesteps $t$ on the generated sample shown. The plot shows the change in loss predicted with the implicit function theorem when linearising the measurement function and when not linearising the measurement, as well as when the model is retrained with data removed. Here, 2500 examples were removed, and each row corresponds to removal of a different subset of 2500 examples.}k         \centering
         \includegraphics[width=\textwidth,trim={0cm 0.0cm 0 0.6cm},clip]{figures/measurement_lin/meas_linearisation_analysis_target_13_removed_examples1_0--diffyscale.pdf}
     \end{subfigure}
    % \includegraphics[width=0.5\linewidth]{}
    \caption{Predicted change in diffusion loss $\mathcal{L}_t$ at different timesteps $t$ on the generated sample shown. The plot shows the change in loss predicted with the implicit function theorem when linearising the measurement function and when not linearising the measurement, as well as when the model is retrained with data removed. Each row corresponds to a different target sample on which the measurement is computed. Here, 1 example was removed.}
    % \label{fig:enter-label}
\end{figure}


% DIFFERENT DAMPING
\begin{figure}[!htb]
    \centering
    \begin{subfigure}[b]{1.0\textwidth}
         \centering
         \includegraphics[width=0.2\textwidth]{figures/measurement_lin/removed_examples1_0.pdf}
    \end{subfigure}
     \begin{subfigure}[b]{1.0\textwidth}
         \centering
         \includegraphics[width=\textwidth,trim={0cm 0.7cm 0 0.0cm},clip]{figures/measurement_lin/meas_linearisation_analysis_target_10_removed_examples1_0--diffyscale.pdf}
     \end{subfigure}
     \begin{subfigure}[b]{1.0\textwidth}
         \centering
         \includegraphics[width=\textwidth,trim={0cm 0.7cm 0 0.6cm},clip]{figures/measurement_lin/meas_linearisation_analysis_target_11_removed_examples1_0--diffyscale.pdf}
     \end{subfigure}
     \begin{subfigure}[b]{1.0\textwidth}
         \centering
         \includegraphics[width=\textwidth,trim={0cm 0.7cm 0 0.6cm},clip]{figures/measurement_lin/meas_linearisation_analysis_target_12_removed_examples1_0--diffyscale.pdf}
     \end{subfigure}
     \begin{subfigure}[b]{1.0\textwidth}
         \centering
         \includegraphics[width=\textwidth,trim={0cm 0.0cm 0 0.6cm},clip]{figures/measurement_lin/meas_linearisation_analysis_target_13_removed_examples1_0--diffyscale.pdf}
     \end{subfigure}
\end{figure}
